Learning Spatially Regularized Correlation Filters for Visual Tracking

Robust and accurate visual tracking is one of the most challenging computer vision problems. Due to the inherent lack of training data, a robust approach for constructing a target appearance model is crucial. Recently, discriminatively learned correlation filters (DCF) have been successfully applied to address this problem for tracking. These methods utilize a periodic assumption of the training samples to efficiently learn a classifier on all patches in the target neighborhood. However, the periodic assumption also introduces unwanted boundary effects, which severely degrade the quality of the tracking model. We propose Spatially Regularized Discriminative Correlation Filters (SRDCF) for tracking. A spatial regularization component is introduced in the learning to penalize correlation filter coefficients depending on their spatial location. Our SRDCF formulation allows the correlation filters to be learned on a significantly larger set of negative training samples, without corrupting the positive samples. We further propose an optimization strategy, based on the iterative Gauss-Seidel method, for efficient online learning of our SRDCF. Experiments are performed on four benchmark datasets: OTB-2013, ALOV++, OTB-2015, and VOT2014. Our approach achieves state-of-the-art results on all four datasets. On OTB-2013 and OTB-2015, we obtain an absolute gain of 8.0% and 8.2% respectively, in mean overlap precision, compared to the best existing trackers.

==> relatedwork.tex <==
\section{Related Work}
The MOSSE tracker \cite{MOSSE2010} and the kernelized extension \cite{Henriques12d} rely on using only grayscale image samples for learning the filter. Later works \cite{DanelljanCVPR14,HenriquesPAMI15,DanelljanBMVC14,Li2014} have gained a notable improvement by learning multi-channel filters on multi-dimensional features, such as HOG \cite{Dalal05} or Color-Names \cite{Weijer09a}. However, to become computationally viable, these approaches rely on harsh approximations of the original multi-channel correlation filter formulation. Typically, a filter is computed for each sample independently and then averaged over time. This may lead to suboptimal learning since all samples are not considered simultaneously in the training. In this work we therefore aim at learning multi-channel correlation filters for the online tracking problem by directly minimizing the associated loss function.
